Arqu\'imedes y las superficies cu\'adricas

A brief review of the history of the conic sections would not be complete without an exhaustively tolerable account of all the things related to the subject that can be found in the extensive work of the wise Archimedes. There is no strong evidence that the Syracusan genius wrote a treatise on Conics separately.

==> Achi1.tex <==
% Encoding: UTF-8

@Article{Holme2010t,
  author    = {Holme, Audun},
  title     = {Greek and Hellenic Geometry},
  journal   = {Geometry},
  year      = {2010},
  month     = jan,
  abstract  = {The word geometry is derived from two Greek words, namely γη, gē, which means earth and μετρου, metron, which means measure. Our sources on early Greek geometry (Fig. 3.1) – and mathematics in general, for that matter – are sparse. Indeed, as far as mathematical contents is concerned we have to rely on the work of the first serious historian of mathematics, namely Eudemus of Rhodes, 350–290 B.C.},
  date      = {2010-01-01},
  doi       = {10.1007/978-3-642-14441-7_3},
  publisher = {Springer},
  url       = {http://dx.doi.org/10.1007/978-3-642-14441-7_3},
}

@Article{Acerbi2019,
  author    = {Acerbi, F.},
  title     = {There is no consequentia mirabilis in Greek mathematics},
  journal   = {Archive for History of Exact Sciences},
  year      = {2019},
  volume    = {73},
  number    = {3},
  pages     = {217},
  month     = may,
  issn      = {1432-0657},
  abstract  = {The paper shows that, contrary to what has been held since the sixteenth-century mathematician Christoph Clavius, there is no application of consequentia mirabilis (CM) in Greek mathematical works. This is shown by means of a detailed discussion of the logical structure of the proofs where CM is allegedly employed. The point is further enlarged to a critical assessment of the unsound methodology applied by many interpreters in seeking for specific logical rules at work in ancient mathematical texts.},
  date      = {2019-05-06},
  doi       = {10.1007/s00407-019-00223-1},
  publisher = {Springer},
  url       = {http://dx.doi.org/10.1007/s00407-019-00223-1},
}

@Article{Risi2016,
  author    = {Risi, Vincenzo},
  title     = {The development of Euclidean axiomatics},
  journal   = {Archive for History of Exact Sciences},
  year      = {2016},
  volume    = {70},
  number    = {6},
  pages     = {591},
  month     = nov,
  issn      = {1432-0657},
  abstract  = {The paper lists several editions of Euclid’s Elements in the Early Modern Age, giving for each of them the axioms and postulates employed to ground elementary mathematics.},
  date      = {2016-11-01},
  doi       = {10.1007/s00407-015-0173-9},
  publisher = {Springer},
  url       = {http://dx.doi.org/10.1007/s00407-015-0173-9},
}

@Article{Masia2016,
  author    = {Masi\`{a}, Ramon},
  title     = {A new reading of Archytas' doubling of the cube and its implications},
  journal   = {Archive for History of Exact Sciences},
  year      = {2016},
  volume    = {70},
  number    = {2},
  pages     = {175},
  month     = mar,
  issn      = {1432-0657},
  abstract  = {The solution attributed to Archytas for the problem of doubling the cube is a landmark of the pre-Euclidean mathematics. This paper offers textual arguments for a new reading of the text of Archytas’ solution for doubling the cube, and an approach to the solution which fits closely with the new reading. The paper also reviews modern attempts to explain the text, which are as complicated as the original, and its connections with some xvi-century mathematical results, without any documented relation to Archytas’ doubling the cube.},
  date      = {2016-03-01},
  doi       = {10.1007/s00407-015-0165-9},
  publisher = {Springer},
  url       = {http://dx.doi.org/10.1007/s00407-015-0165-9},
}

@Article{Masia2015,
  author    = {Masi\`{a}, Ramon},
  title     = {On dating Hero of Alexandria},
  journal   = {Archive for History of Exact Sciences},
  year      = {2015},
  volume    = {69},
  number    = {3},
  pages     = {231},
  month     = may,
  issn      = {1432-0657},
  abstract  = {The dating of Hero of Alexandria has been linked with the lunar eclipse of March 13, ad 62, since Otto Neugebauer discovered that this eclipse is the only one that can fit the one described in Hero’s Dioptra 35. Although only a number of scholars claim that Hero himself observed the eclipse, almost all of them take Neugebauer’s identification for granted. We use statistical and linguistic methods to criticize this assumption: all indices we have found point to the fact that the eclipse was merely invented as an example and, for that reason, that it cannot be used to determine Hero’s life span.},
  date      = {2015-05-01},
  doi       = {10.1007/s00407-014-0148-2},
  publisher = {Springer},
  url       = {http://dx.doi.org/10.1007/s00407-014-0148-2},
}

@Article{Corry2013,
  author    = {Corry, Leo},
  title     = {Geometry and arithmetic in the medieval traditions of Euclid's Elements: a view from Book II},
  journal   = {Archive for History of Exact Sciences},
  year      = {2013},
  volume    = {67},
  number    = {6},
  pages     = {637},
  month     = nov,
  issn      = {1432-0657},
  abstract  = {This article explores the changing relationships between geometric and arithmetic ideas in medieval Europe mathematics, as reflected via the propositions of Book II of Euclid’s Elements. Of particular interest is the way in which some medieval treatises organically incorporated into the body of arithmetic results that were formulated in Book II and originally conceived in a purely geometric context. Eventually, in the Campanus version of the Elements these results were reincorporated into the arithmetic books of the Euclidean treatise. Thus, while most of the Latin versions of the Elements had duly preserved the purely geometric spirit of Euclid’s original, the specific text that played the most prominent role in the initial passage of the Elements from manuscript to print—i.e., Campanus’ version—followed a different approach. On the one hand, Book II itself continued to appear there as a purely geometric text. On the other hand, the first ten results of Book II could now be seen also as possiblytranslatable into arithmetic, and in many cases even as inseparably associated with their arithmetic representation.},
  date      = {2013-11-01},
  doi       = {10.1007/s00407-013-0121-5},
  publisher = {Springer},
  url       = {http://dx.doi.org/10.1007/s00407-013-0121-5},
}

@Article{Acerbi2011,
  author    = {Acerbi, Fabio},
  title     = {The geometry of burning mirrors in Greek antiquity. Analysis, heuristic, projections, lemmatic fragmentation},
  journal   = {Archive for History of Exact Sciences},
  year      = {2011},
  volume    = {65},
  number    = {5},
  pages     = {471},
  month     = sep,
  issn      = {1432-0657},
  abstract  = {The article analyzes in detail the assumptions and the proofs typical of the research field of the geometry of burning mirrors. It emphasizes the role of two propositions of the Archimedean Quadratura parabolae, never brought to bear on this subject, and of a complex system of projections reducing a sumptōma of a parabola to some specific linear lemmas. On the grounds of this case-study, the much-debated problem of the heuristic role of analysis is also discussed.},
  date      = {2011-09-01},
  doi       = {10.1007/s00407-010-0076-8},
  publisher = {Springer},
  url       = {http://dx.doi.org/10.1007/s00407-010-0076-8},
}

@Article{Acerbi2011a,
  author    = {Acerbi, Fabio},
  title     = {The language of the Givens: its forms and its use as a deductive tool in Greek mathematics},
  journal   = {Archive for History of Exact Sciences},
  year      = {2011},
  volume    = {65},
  number    = {2},
  pages     = {119},
  month     = mar,
  issn      = {1432-0657},
  abstract  = {The aim of this article is to present and discuss the language of the «givens», a typical stylistic resource of Greek mathematics and one of the major features of the proof format of analysis and synthesis. I shall analyze its expressive function and its peculiarities, as well as its general role as a deductive tool, explaining at the same time its particular applications in subgenres of a geometrical proposition like the locus theorems and the so-called «porisms». The main interpretative theses of this study are the following: the language of the «givens» (1) is the standard idiom in which “existence and uniqueness” of a mathematical object was proved, (2) was conceived as an unified framework reducing to a strictly deductive format disparate argumentative steps such as deductions, constructions, and calculations.},
  date      = {2011-03-01},
  doi       = {10.1007/s00407-010-0072-z},
  publisher = {Springer},
  url       = {http://dx.doi.org/10.1007/s00407-010-0072-z},
}

@Article{Acerbi2009,
  author    = {Acerbi, Fabio},
  title     = {The meaning of \textgreek{Plasmatik\A{o}n} in Diophantus Arithmetica},
  journal   = {Archive for History of Exact Sciences},
  year      = {2009},
  volume    = {63},
  number    = {1},
  pages     = {5},
  month     = jan,
  issn      = {1432-0657},
  abstract  = {Three problems in book I of Diophantus’ Arithmetica contain the adjective plasmatikon, that appears to qualify an implicit reference to some theorems in Elements, book II. The translation and meaning of the adjective sparked a long-lasting controversy that has become a nonnegligible aspect of the debate about the possibility of interpreting Diophantus’ approach and, more generally, Greek mathematics in algebraic terms. The correct interpretation of the word, a technical term in the Greek rhetorical tradition that perfectly fits the context in which it is inserted in the Arithmetica, entails that Diophantus’ text contained no (implicit) reference to Euclid’s Elements. The clause containing the adjective turns out to be a later interpolation, that cannot be used to support any algebraic interpretation of the Arithmetica.},
  date      = {2009-01-01},
  doi       = {10.1007/s00407-008-0028-8},
  publisher = {Springer},
  url       = {http://dx.doi.org/10.1007/s00407-008-0028-8},
}

@Article{Hoeyrup2019,
  author        = {H{\o}yrup, Jens},
  title         = {From the Practice of Explanation to the Ideology of Demonstration: An Informal Essay},
  journal       = {Interfaces between Mathematical Practices and Mathematical Education},
  year          = {2019},
  month         = jan,
  __markedentry = {[laboratorio:]},
  abstract      = {The following discusses the practice of mathematical argument or demonstration—at first based on what I shall speak of as “the locally obvious”, that is, presuppositions which the interlocutor—or, in case of writing, the imagined or “model” reader—will accept as obvious; next in its interaction with critique, investigation of the conditions for the validity of the seemingly obvious as well as the limits of this validity. This is done, in part through analysis of material produced within late medieval Italian abbacus culture, in part from a perspective offered by the Old Babylonian mathematical corpus—both sufficiently distant from what we are familiar with to make phenomena visible which in our daily life go as unnoticed as the air we breathe; that is, they allow Verfremdung. These tools are then applied to the development from argued procedure toward axiomatics in ancient Greece, from the mid-fifth to the mid-third century bce. Finally is discussed the further development of ancient demonstrative mathematics, when axiomatization, at first a practice, then a norm, in the end became an ideology. The whole is rounded off by a few polemical remarks about present-day beliefs concerning the character of mathematics.},
  date          = {2019-01-01},
  doi           = {10.1007/978-3-030-01617-3_2},
  publisher     = {Springer},
  url           = {http://dx.doi.org/10.1007/978-3-030-01617-3_2},
}

@Article{Rabouin2015,
  author        = {Rabouin, David},
  title         = {Proclus' Conception of Geometric Space and Its Actuality},
  journal       = {Mathematizing Space},
  year          = {2015},
  month         = jan,
  __markedentry = {[laboratorio:]},
  abstract      = {The main aim of this paper is to present ProclusProclus’ philosophy of geometric extension not so much from the point of view of what he says about it as what he does with it. I will henceforth pay particular attention to the role of spatial configurations in the practice which he describes. My motivations are twofold. First, although ProclusProclus’ philosophy of geometry has received quite a lot of attention in the scholarship, this attention has remained mainly inspired by the philosophical doctrine expounded in the Prologues. It did not engage much, at least in a systematic way, with the material given in the actual commentary of EuclidEuclid’s propositions and the mathematical practice there described. As a consequence, the complexity and the flexibility of ProclusProclus’ views on the geometric imagination were not always well rendered. I would like to complete existing descriptions by paying more attention to these details, although, as I will indicate, they may sometimes introduce important nuances, if not tensions, in the philosophical system. Second, ProclusProclus provides indications throughout his commentary about the geometric practice which go far beyond his own specific philosophical agenda. He deals, for example, with objections that other mathematicians and philosophers raised against EuclidEuclid’s proofs. These objections, which sometimes stem from views opposite to his own (typically, Epicurean objections of an “empiricist” flavor), were taken seriously enough to ask for answers which ProclusProclus also mentions (or sometimes even initiates). For the modern reader, these passages are precious because they provide, by contrast, testimonies about certain conditions of the practice which seem to have been accepted by the various interlocutors (whatever their philosophical background may have been). I would like to reconstitute some of these conditions and compare these reconstructions with recent works dealing with ancient Greek geometric practice, especially as regards the use of diagrams.},
  date          = {2015-01-01},
  doi           = {10.1007/978-3-319-12102-4_5},
  publisher     = {Springer},
  url           = {http://dx.doi.org/10.1007/978-3-319-12102-4_5},
}

@Article{Sidoli2014,
  author        = {Sidoli, Nathan},
  title         = {Research on Ancient Greek Mathematical Sciences, 1998-2012},
  journal       = {From Alexandria, Through Baghdad},
  year          = {2014},
  month         = jan,
  __markedentry = {[laboratorio:]},
  abstract      = {This survey deals with research in ancient Greek mathematics and, to a lesser extent, mathematical sciences in the long first decade of the 21st century. It is modeled on the two foregoing surveys by J.L. Berggren and K. Saito and gives my personal appraisal of the most important work and trends of the last years, with no attempt to be exhaustive.},
  date          = {2014-01-01},
  doi           = {10.1007/978-3-642-36736-6_3},
  publisher     = {Springer},
  url           = {http://dx.doi.org/10.1007/978-3-642-36736-6_3},
}

@Article{Christianidis2013,
  author        = {Christianidis, Jean},
  title         = {The Archimedes palimpsest: the definitive edition},
  journal       = {Metascience},
  year          = {2013},
  volume        = {22},
  number        = {1},
  pages         = {137},
  month         = mar,
  issn          = {1467-9981},
  __markedentry = {[laboratorio:]},
  date          = {2013-03-01},
  doi           = {10.1007/s11016-012-9682-1},
  publisher     = {Springer},
  url           = {http://dx.doi.org/10.1007/s11016-012-9682-1},
}

@Article{Sidoli2018a,
  author        = {Sidoli, Nathan},
  title         = {The concept of given in Greek mathematics},
  journal       = {Archive for History of Exact Sciences},
  year          = {2018},
  volume        = {72},
  number        = {4},
  pages         = {353},
  month         = jul,
  issn          = {1432-0657},
  __markedentry = {[laboratorio:6]},
  abstract      = {This paper is a contribution to our understanding of the technical concept of given in Greek mathematical texts. By working through mathematical arguments by Menaechmus, Euclid, Apollonius, Heron and Ptolemy, I elucidate the meaning of given in various mathematical practices. I next show how the concept of given is related to the terms discussed by Marinus in his philosophical discussion of Euclid’s Data. I will argue that what is given does not simply exist, but can be unproblematically assumed or produced through some effective procedure. Arguments by givens are shown to be general claims about constructibility and computability. The claim that an object is given is related to our concept of an assignment—what is given is available in some uniquely determined, or determinable, way for future mathematical work.},
  date          = {2018-07-01},
  doi           = {10.1007/s00407-018-0211-5},
  publisher     = {Springer},
  url           = {http://dx.doi.org/10.1007/s00407-018-0211-5},
}

@Article{Thomas2018,
  author        = {Thomas, R. S. D.},
  title         = {The Definitions and Theorems of the Spherics of Theodosios},
  journal       = {Research in History and Philosophy of Mathematics},
  year          = {2018},
  month         = jan,
  __markedentry = {[laboratorio:6]},
  abstract      = {My journal article abbreviation of Euclid’s Phenomena with Len Berggren shows what the book says to those that don’t need or want the whole treatise. Its most important part is a list of the enunciations of the theorems as the obvious way to express the contents. This is a summary of the Spherics of Theodosios for “those that don’t need or want the whole treatise”. That summary is the second long section of this paper. The first section explains why, with examples, the summary cannot be just “a list of the enunciations of the theorems”.},
  date          = {2018-01-01},
  doi           = {10.1007/978-3-319-90983-7_1},
  publisher     = {Springer},
  url           = {http://dx.doi.org/10.1007/978-3-319-90983-7_1},
}

@Article{Saito2014,
  author        = {Saito, Ken and Napolitani, Pier Daniele},
  title         = {Reading the Lost Folia of the Archimedean Palimpsest: The Last Proposition of the Method},
  journal       = {From Alexandria, Through Baghdad},
  year          = {2014},
  month         = jan,
  __markedentry = {[laboratorio:6]},
  abstract      = {We examine the determination of the volume of solids by means of a virtual balance, in Archimedes’ Method a work preserved only in the Archimedes palimpsest.We concentrate on the intersection of two cylinders, whose volume is correctly stated in the preface, although the folia containing the proof are lost.},
  date          = {2014-01-01},
  doi           = {10.1007/978-3-642-36736-6_10},
  publisher     = {Springer},
  url           = {http://dx.doi.org/10.1007/978-3-642-36736-6_10},
}

@Article{Lorch2014,
  author        = {Lorch, Richard},
  title         = {The Second Arabic Translation of Theodosius' Sphaerica},
  journal       = {From Alexandria, Through Baghdad},
  year          = {2014},
  month         = jan,
  __markedentry = {[laboratorio:6]},
  abstract      = {From a short comparison of terminology it is suggested that the Arabic text of Theodosius' Sphtzerica carried by two manuscripts in Hebrew script is a translation different from the one translated by Gerard of Cremona into Latin. An edition of a lemma for Proposition 11!.11 inter alia supports the hypothesis that this translation is the basis of Moses b. Tibbon's Hebrew version.},
  date          = {2014-01-01},
  doi           = {10.1007/978-3-642-36736-6_13},
  publisher     = {Springer},
  url           = {http://dx.doi.org/10.1007/978-3-642-36736-6_13},
}

@Article{Bernard2014,
  author        = {Bernard, Alain and Proust, Christine and Ross, Micah},
  title         = {Mathematics Education in Antiquity},
  journal       = {Handbook on the History of Mathematics Education},
  year          = {2014},
  month         = jan,
  __markedentry = {[laboratorio:6]},
  abstract      = {This chapter is derived from highly heterogeneous sources both in their nature and in their geographic and chronological distribution. These sources represent different environments and refer to different cultural and institutional codes. Whereas ancient sources do not describe a coherent picture of teaching mathematics in Antiquity, some details from the better documented educational contexts of Mesopotamia, Egypt, and the Greco-Roman World provide impressionistic insight into these traditions. This approach shows that modern knowledge of these contexts is limited and that even the kinds of questions framing the topic depend strictly on the nature of the surviving sources.},
  date          = {2014-01-01},
  doi           = {10.1007/978-1-4614-9155-2_3},
  publisher     = {Springer},
  url           = {http://dx.doi.org/10.1007/978-1-4614-9155-2_3},
}

@Article{Saito2014a,
  author        = {Saito, Ken},
  title         = {Mathematical Reconstructions Out, Textual Studies In: 30 Years in the Historiography of Greek Mathematics [1998]},
  journal       = {From Alexandria, Through Baghdad},
  year          = {2014},
  month         = jan,
  __markedentry = {[laboratorio:6]},
  abstract      = {Thirty years ago, at the end of the sixties, the history of Greek mathematics was considered an almost dosed subject, just like physics was at the turn of the twentieth century. People felt that they had constructed a definitive picture of the essence of Greek mathematics, even though some details remained unclear due to irrecoverable document losses. Critical editions had been established, mainly by Heiberg, while two of the great scholars of the history of Greek mathematics, Tannery and Zeuthen, had built on this material. Then, the standard book [Heath 1921] brought much of this material together. Through his discoveries in Mesopotamian mathematics, Neugebauer was led to think that he had given substance to legends about the Oriental origin of Greek mathematics. Originally published in Dutch in 1950, the book [van der Waerden 1954] reflected scholars' self-confidence in this period.},
  date          = {2014-01-01},
  doi           = {10.1007/978-3-642-36736-6_2},
  publisher     = {Springer},
  url           = {http://dx.doi.org/10.1007/978-3-642-36736-6_2},
}

@Article{Berggren2014,
  author        = {Berggren, J. Lennart},
  title         = {History of Greek Mathematics: A Survey of Recent Research [1984]},
  journal       = {From Alexandria, Through Baghdad},
  year          = {2014},
  month         = jan,
  __markedentry = {[laboratorio:6]},
  abstract      = {This survey reviews research in four areas of the history of Greek mathematics: (1) methods in Greek mathematics (the axiomatic method, the method of analysis, and geometric algebra); (2) proportion and the theory of irrationals (controversies over the origins of the theory of incommensurabies); (3) Archimedes (aspects of controversies over his life and works); and (4) Greek mathematical methods (including discussion of Ptolemy's work, connections between Greek and Indian mathematics, the significance of Greek mathematical papyri, Arabic texts, and even archaeological investigations of scientific instruments).},
  date          = {2014-01-01},
  doi           = {10.1007/978-3-642-36736-6_1},
  publisher     = {Springer},
  url           = {http://dx.doi.org/10.1007/978-3-642-36736-6_1},
}

@Article{Berggren2014a,
  author        = {Berggren, J. Lennart},
  title         = {History of Mathematics in the Islamic World: The Present State of the Art [1985]},
  journal       = {From Alexandria, Through Baghdad},
  year          = {2014},
  month         = jan,
  __markedentry = {[laboratorio:6]},
  abstract      = {In recent years, many discoveries in the history of Islamic mathematics have not been reported outside the specialist literature, even though they raise issues of interest to a larger audience. Thus, our aim in writing this survey is to provide to scholars of Islamic culture an account of the major themes and discoveries of the last decade of research on the history of mathematics in the Islamic world. However, the subject of mathematics comprised much more than what a modern mathematician might think of as belonging to mathematics, so our survey is an overview of what may best be called the "mathematical sciences" in Islam; that is, in addition to such topics as arithmetic, algebra, and geometry we will also be interested in mechanics, optics, and mathematical instruments.},
  date          = {2014-01-01},
  doi           = {10.1007/978-3-642-36736-6_4},
  publisher     = {Springer},
  url           = {http://dx.doi.org/10.1007/978-3-642-36736-6_4},
}

@Article{Berggren2014b,
  author        = {Berggren, J. Lennart},
  title         = {Mathematics and Her Sisters in Medieval Islam: A Selective Review of Work Done from 1985 to 1995 [1997]},
  journal       = {From Alexandria, Through Baghdad},
  year          = {2014},
  month         = jan,
  __markedentry = {[laboratorio:6]},
  abstract      = {This paper surveys work done over the past decade, largely in Western Europe and North America, in the history of the mathematical sciences as practiced in medieval Islam from central Asia to Spain. Among the major topics covered, in addition to the usual branches of mathematics, are mathematical geography, astronomy, and optics. We have also given accounts of some current debates on the interpretation ofimportant texts and, in addition, we havesu rveyed some of the literature dealing with the interrelation of mathematics and society in medieval Islam.},
  date          = {2014-01-01},
  doi           = {10.1007/978-3-642-36736-6_5},
  publisher     = {Springer},
  url           = {http://dx.doi.org/10.1007/978-3-642-36736-6_5},
}

@Article{Sidoli2009,
  author        = {Sidoli, Nathan and Saito, Ken},
  title         = {The Role of Geometrical Construction in Theodosius's Spherics},
  journal       = {Archive for History of Exact Sciences},
  year          = {2009},
  volume        = {63},
  number        = {6},
  pages         = {581},
  month         = aug,
  issn          = {1432-0657},
  __markedentry = {[laboratorio:6]},
  abstract      = {This paper is a contribution to our understanding of the constructive nature of Greek geometry. By studying the role of constructive processes in Theodoius’s Spherics, we uncover a difference in the function of constructions and problems in the deductive framework of Greek mathematics. In particular, we show that geometric problems originated in the practical issues involved in actually making diagrams, whereas constructions are abstractions of these processes that are used to introduce objects not given at the outset, so that their properties can be used in the argument. We conclude by discussing, more generally, ancient Greek interests in the practical methods of producing diagrams.},
  date          = {2009-08-11},
  doi           = {10.1007/s00407-009-0045-2},
  publisher     = {Springer},
  url           = {http://dx.doi.org/10.1007/s00407-009-0045-2},
}

@Comment{jabref-meta: databaseType:bibtex;}

